Combination of Site-Wide and Real-Time Optimization for the Control of Systems of Electrolyzers

The rapid expansion of renewable energy sources has introduced significant volatility and unpredictability in the energy supply chain, necessitating advanced control strategies to ensure grid stability and reliability. Green hydrogen production via electrolysis offers a viable solution for converting and storing this volatile renewable energy. However, the inherent fluctuations of renewable energy sources present challenges for consistent utilization and integration of green hydrogen. This work proposes a two-stage optimization approach, combining site-wide optimization and real-time optimization for managing systems of electrolyzers. By adapting an existing static optimization model, dual use is achieved in both site-wide optimization and real-time optimization. The hierarchical optimization structure, characterized by distinct temporal resolutions, enables effective responses to both dynamic changes and long-term trends. The side-wide optimization layer generates long-term plans based on forecast data, while the real-time optimization layer refines these plans in real-time, accommodating immediate fluctuations and ensuring efficient operation. The results from the case study on a system of electrolyzers demonstrate the method's effectiveness in aligning electrolyzer operation with actual availability of renewable energy. This approach offers a robust framework for optimizing the operation of electrolyzers but also other types of flexible energy resources, contributing to sustainable and economically viable energy management.

==> acronyms.tex <==
%alphabetisch anordnen
%https://www.namsu.de/Extra/pakete/Acronym.html
% Beispiel: \acro{1}[2]{3}
% 1: so wird die Abkürzung im Text mit \ac{1} aufgerufen. 
% beim ersten Aufruf steht dann da 3 (2), also
% 2: richtige Schreibweise der Abkürzung
% 3: Langform der Abkürzung
% -- A ------------------------------------------------------------------------------------------------------%
\acro{AAS}{Asset Administration Shell}
\acroplural{AAS}{Asset Administration Shells}
\acro{ADMM}{Alternating Direction Method of Multipliers}
\acro{AEL}{Alkaline Electrolysis}
\acro{AEM}{Anion Exchange Membrane Electrolysis}
\acro{AI}{Artificial Intelligence}
% -- B ------------------------------------------------------------------------------------------------------%
% -- C ------------------------------------------------------------------------------------------------------%
\acro{CAEX}{Computer Aided Engineering Exchange}
\acro{CapEx}{Capital Expenditure}
% -- D ------------------------------------------------------------------------------------------------------%
\acro{DCS}{Distributed Control System}
\acro{2DECS}{Development Approach for DEcentralised Control Systems}
\acro{DSM}{Demand Side Management}
\acro{DT}{Digital Twin}
\acroplural{DT}[DTs]{Digital Twins}
% -- E ------------------------------------------------------------------------------------------------------%
\acro{XML}{Extensible Markup Language}
% -- F ------------------------------------------------------------------------------------------------------%
% -- G ------------------------------------------------------------------------------------------------------%
% -- H ------------------------------------------------------------------------------------------------------%
\acro{HTEL}{High-Temperature Electrolysis}
\acro{H2PC}{H2-Production-Coordination}
% -- I ------------------------------------------------------------------------------------------------------%
\acro{ICPS}{Industrial Cyber-Physical Production System}
\acroplural{ICPS}{Industrial Cyber-Physical Production Systems}
% -- J ------------------------------------------------------------------------------------------------------%
% -- K ------------------------------------------------------------------------------------------------------%
% -- L ------------------------------------------------------------------------------------------------------%
\acro{LCOH}{Levelized Cost of Hydrogen}
% -- M ------------------------------------------------------------------------------------------------------%
\acro{MAS}{Multi-Agent System}
\acroplural{MAS}[MASs]{Multi-Agent Systems}
\acro{milp}[MILP]{Mixed-integer linear programming}
\acro{mLCOH}{Marginal Levelized Cost of Hydrogen}
\acro{MPC}{Model Predictive Control}
\acro{MTP}{Module Type Package}
% -- N ------------------------------------------------------------------------------------------------------%
% -- O ------------------------------------------------------------------------------------------------------%
\acro{OD}{Orchestration Designer}
\acro{OM}{Operation \& Maintenance}
\acro{OpEx}{Operational Expenditure}
% -- P ------------------------------------------------------------------------------------------------------%
\acro{PEA}{Process Equipment Assembly}
\acroplural{PEA}[PEAs]{Process Equipment Assemblies}
\acro{PEA-S}{PEA-Scheduling}
\acro{PEM}{Proton Exchange Membrane Electrolysis}
\acro{PID}{Proportional-Integral-Differential}
\acro{pla}[PLA]{Piecewise linear approximation}
\acro{POL}{Process Orchestration Layer}
\acroplural{POL}[POLs]{Process Orchestration Layers}
\acro{P2O}{Process2Order}
% -- Q ------------------------------------------------------------------------------------------------------%
% -- R ------------------------------------------------------------------------------------------------------%
\acro{REQ}{Requirement}
\acroplural{REQ}[REQs]{Requirements}
\acro{RE}{Renewable Energy}
\acro{RTO}{Real-Time Optimization}
% -- S ------------------------------------------------------------------------------------------------------%
\acro{SIP}{Standard Integration Profile}
\acro{soc}[SOC]{state of charge}
\acro{SoS}{Set of Setpoints}
\acro{SWO}{Site-wide Optimization}
% -- T ------------------------------------------------------------------------------------------------------%
% -- U ------------------------------------------------------------------------------------------------------%
% -- V ------------------------------------------------------------------------------------------------------%
% -- W ------------------------------------------------------------------------------------------------------%
% -- X ------------------------------------------------------------------------------------------------------%
% -- Y ------------------------------------------------------------------------------------------------------%
% -- Z ------------------------------------------------------------------------------------------------------%

==> figures/algo_transform.tex <==
\begin{algorithm}[h]
\footnotesize
\DontPrintSemicolon
\caption{Transformation of Existing Model}
\label{alg:transform}
\KwData{OptimizationModel \textit{optModel}}
\KwResult{RTOModel \textit{rtoModel}}
\SetKwFunction{transModel}{transformModel}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\transModel{optModel}}{
rtoModel $\gets$ optModel\; 
rtoModel.addConstraints(optModel.decisionVariables())\;
\Return rtoModel\;
}
\end{algorithm}
